A Comprehensive Analysis on the Learning Curve in Kernel Ridge Regression

This paper conducts a comprehensive study of the learning curves of kernel ridge regression (KRR) under minimal assumptions. Our contributions are three-fold: 1) we analyze the role of key properties of the kernel, such as its spectral eigen-decay, the characteristics of the eigenfunctions, and the smoothness of the kernel; 2) we demonstrate the validity of the Gaussian Equivalent Property (GEP), which states that the generalization performance of KRR remains the same when the whitened features are replaced by standard Gaussian vectors, thereby shedding light on the success of previous analyzes under the Gaussian Design Assumption; 3) we derive novel bounds that improve over existing bounds across a broad range of setting such as (in)dependent feature vectors and various combinations of eigen-decay rates in the over/underparameterized regimes.

==> section/discussion.tex <==
In this section, we elaborate further on the results presented in this paper, and discuss their implications in relation to the three questions raised in Section \ref{section:introduction}.


\subsection{Proof Sketch}

All the above results can be proven under the same set of assumptions and proof techniques. In more details:
\begin{enumerate}
    \item The starting point of the analysis relies on some \emph{Master inequalities}:
    \begin{align*}
        \B  
            &\leq 
            \underbrace{\textcolor{gray}{\left(\frac{1+\rho^2 \zeta^2 \xi^{-1}+\rho}{\delta}\right)}}_{\text{constant}}
            \overbrace{\|\th_{>k}^*\|_{\Si_{>k}}^2}^{\text{target's tail}}
            + 
            \underbrace{\textcolor{gray}{(\zeta^2\xi^{-2}+\rho \zeta^2\xi^{-1})}}_{\text{constant}}
            \overbrace{\frac{s_1(\A_k)^2}{n^2} }^{\approx (\lambda_k +\lambda)^2} 
            \underbrace{\norm{\th^*_{\leq k}}{\Si_{\leq k}^{-1}}^2}_{\text{target's head}};\\
        \V 
        &\leq
        \underbrace{\sigma^2}_{\text{noise level}} 
        \textcolor{gray}{\rho^2}
        \left(
        \underbrace{\textcolor{gray}{\zeta^2\xi^{-1}}}_{\text{constant}}
        \frac{k}{n}
        +
        \underbrace{\textcolor{gray}{\frac{\tr[\Z_{>k}\Si_{>k}^2\Z_{>k}^\top]}{n\tr[\Si_{>k}^2]} \frac{r_k(\Si)^2}{nR_k(\Si)}}}_{=\bigo{}{\frac{k}{n}}}
        \right).
    \end{align*}

\textcolor{blue}{I would use a big O notation to hide the constants in above inequalities. We should also say it's valid for any $k$ and define important quantities, e.g. $\A_k$.}
    
    Intuitively, the Master inequalities bounds the bias $\B$ and the variance $\V$ terms in terms of the kernel eigen-spectrum as well as the target coefficients, given that $\rho\eqdef$ the condition number of the truncated kernel matrix $\A_k$ is bounded.
    See Section \ref{section:non_asymptotic_bound} for the details of the notations and the proof of the Master inequalities.
    \item We first study the properties of the features using concentration results under Assumptions \ref{assumption:GF} or \ref{assumption:IF} (see Section \ref{section:concentration});
    \item Using the above result, we bound the condition number of the (truncated) kernel matrix (see Section \ref{section:concentration}) as in \cite{barzilai2023generalization, cheng2024characterizing}, which will be used to bound the test error in the next step;
    \item Combining the bound of the condition number with the result from \cite{bartlett2020benign, tsigler2023benign}, which we call the \emph{Master inequalities}, we can compute the test error bound for various settings (see Section \ref{section:proof});
    \item In the over-parameterized regime, we know most of the bounds derived are tight according to \cite{li2023kernel, li2023on, long2024duality}, and we also modify a proposition from \cite{li2023on} to improve the bound from \cite{barzilai2023generalization} (see Figure \ref{fig:phase_diagram});
    \item In the under-parameterized regime, the Master inequalities also gives an upper bound for $\B$ and $\V$, which might not be tight if the ridge $\lambda$ is strong. However, we present another way to obtain tight bounds without the Master inequalities (see Section \ref{section:under_parameterized} for more details).
\end{enumerate}
% We summarize the proof techniques by a flowchart in Figure \ref{fig:flowchart}, and thus we can answer the second question we raised in Section \ref{section:introduction}:
% \begin{center}
%     \textit{Is there a unifying theory under various settings and minimal assumptions?}\\
%     \textbf{Yes.}
% \end{center}





\subsection{Independent and Generic Features} \label{subsection:IGF}
Table \ref{tab:over_parameterized} indicates that the test error exhibits the same upper bound with either independent or generic features under strong ridge conditions in the over-parameterized regime. This similarity arises from the bounds in both cases being derived from the Master inequalities. However, under weak ridge conditions, the empirical kernel spectrum displays qualitative differences, as reported in \cite{barzilai2023generalization, cheng2024characterizing}. From Figure \ref{fig:overfitting}, we can see that $\V=\bigo{}{1}$ with Laplacian kernel in the left plot and $\V$ diverges with neural tangent kernel (with 1 hidden layer) in the right plot. Hence under weak ridge and polynomial eigen-decay, the case distinction of the bound
\begin{equation*}
    \V
    =
    \begin{cases}
        \bigtheta{}{\sigma^2} ,& \text{Assumption \ref{assumption:IF} holds}, \\
        \bigo{}{\sigma^2n^{2a}} ,& \text{Assumption \ref{assumption:GF} holds}
    \end{cases}
\end{equation*}
in Table \ref{tab:over_parameterized} is necessary, as Assumption \ref{assumption:GF} includes the cases of Gaussian Design \ref{assumption:GD} (or more generally independent features \ref{assumption:IF}) and Laplacian kernel which yields $\V=\bigtheta{}{1}$, the so-called tempered overfitting from \cite{mallinar2022benign}; as well as the case of neural tangetn kernel (NTK) which yields $\V\xrightarrow[]{n\to\infty}\infty$, teh so-called catastrophic overfitting. In particular, our proof shows that the Gaussian Equivalent Property (GEP) does not hold under weak ridge. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{pictures/variance_Laplacian.png}
    \includegraphics[width=0.45\linewidth]{pictures/variance_NTK_L=1.png}
    \caption{Under weak ridge, kernels with polynomial eigen-decay can have qualitative different asymptotic behaviours. See Section \ref{section:experiment} for more details.}
    \label{fig:overfitting}
\end{figure}


%Hence, for polynomial eigen-decay, the bounds differ: with independent features, we still obtain tight bounds for both $\B$ and $\V$, while with generic features, the upper bound is looser. Conversely, for exponential decay, we achieve a tight upper bound of $\B$ for both types of features only under the condition that $s > 1$. We omit the upper bound of $\V$ because even for independent features, the variance is known to be unbounded, a phenomenon referred to as catastrophic overfitting in \cite{mallinar2022benign}.

We are now prepared to address the first question posed in Section \ref{section:introduction}:

\begin{center}
\textit{Q1: When and why does the Gaussian Equivalence Property (GEP) exist?}\\
\textbf{The Master inequalities provide the same non-asymptotic bounds for both cases under a strong ridge. \textcolor{red}{However, GEP does not exists under weak ridge!}}
\end{center}

In particular, our work implies that previous works \cite{bordelon2020spectrum, cui2021generalization, loureiro2021learning, simon2023eigenlearning, mallinar2022benign} under Gaussian Design assumption \ref{assumption:GD} can be applied only when the ridge is strong.
Upon finalizing the preparation for this paper, we became aware of concurrent research conducted by \cite{gavrilopoulos2024geometrical}, which also concerns the Gaussian Equivalence Property (GEP) in the non-asymptotic setting. For more comparison between their assumptions and ours, we refer the reader to Section \ref{section:assumptions}.


\subsection{Importance of Ridge}

To address the second question posed in Section \ref{section:introduction}, it is evident that in either the under-parameterized setting with any ridge (see Table \ref{tab:under_parameterized}) or the over-parameterized regime with a strong ridge (see Table \ref{tab:over_parameterized}), the bounds for both $\B$ and $\V$ remain the same, irrespective of the features:
\begin{center}
    \textit{Q2: Under which conditions can one tease apart role of the eigen-decay in the generalization performance?}\\
    \textbf{Either (i) in under-parameterized setting; or (ii) with strong ridge in over-parameterized regime.}
\end{center}

Several results \cite{rosasco2010learning, long2024duality, misiakiewicz2024nonasymptotic} have suggested that the test error bound can be characterized by the covariance spectrum $\Si$, but they implicitly require the ridge $\lambda>0$ to be larger than some metric. This paper clearly demonstrates the necessity of the presence of a strong ridge in such analyses.

Notably, in the lower right corner in Table \ref{tab:over_parameterized}, we acknowledge the issue of catastrophic overfitting in kernel interpolation with exponential eigen-decay \cite{mallinar2022benign, cheng2024characterizing}, where there is no reasonable upper bound for the variance term $\V$. 

Under weak ridge, the independence of features also play an important role on. See Subsection \ref{subsection:overfitting} for more details.

\subsection{Tempered versus Catastrophic Overfitting} \label{subsection:overfitting}
The weak ridge setting also includes the so-called ridgeless or interpolation case, where the regressor $\hat{f}$ is the minimum norm interpolant of the outputs. In this case with polynomial eigen-decay, our result with independent features ensures the overfitting to be tempered, recovering and extending the results from \cite{cui2021generalization, mallinar2022benign, cheng2024characterizing}; however, as reported in \cite{barzilai2023generalization}, the overfitting can be catastrophic in a kernel setting. Also, \cite{haas2023mind, li2023kernel} only showed the inconsistency of KRR by providing a positive constant lower bound of $\V$ where the upper bound is not discussed. 

\subsection{Polynomial versus Exponential Eigen-Decay}

From Table \ref{tab:over_parameterized}, we can see that the eigen-decay also affects the test error qualitatively.

\paragraph{Under strong ridge}
As mentioned in \cite{long2024duality}, the bias term $\B$ decays polynomially (or resp. exponentially), when the eigen-decay is polynomial (or resp. exponential). However, we prove that $\V$ decays only polynomially at a rate at most $\bigo{}{\frac{1}{n}}$, regardless of the eigen-decay. Hence, in a noisy setting with polynomial eigen-decay, one can find an optimal ridge $\lambda=\bigtheta{n}{n^{-\frac{1+a}{(1+a)\tilde{s}+1}}}$ to balance both terms $\B$ and $\V$ as in \cite{cui2021generalization, li2023on}.
%\footnote{Recall that $\lambda_k=\bigtheta{k}{k^{-1-a}}$, $|\theta^*_k|=\bigtheta{k}{k^{-r}}$ for some $a,r>0$, $\lambda=\bigtheta{n}{n^{-b}}$ for some $b\in(0,1+a)$, then we can choose $s=\frac{2r}{a+1}$ and let $\Tilde{s}\eqdef\min\{s,2\}$. See Section \ref{section:assumptions} for details. Assume the noise level $\sigma^2=\bigtheta{n}{1}$ is independent to $n$.}
In contrast, in noisy settings with exponential eigen-decay, $\V$ dominates the test error.

\paragraph{Under weak ridge} The variance term $\V$ is omitted in the case with exponential eigen-decay due to the so-called catastrophic overfitting phenomenon observed in \cite{mallinar2022benign}. However, with polynomial eigen-decay, $\V$ remains bounded polynomially and exhibits the so-called tempered overfitting phenomenon, particularly with independent features.



\subsection{Improved upper bound} \label{subsection:improved_ub}
During our research, we discovered that we can improve the upper bound of $\B$ in the over-parameterized regime with polynomial decay, weak ridge and Assumption \ref{assumption:GF} by modifying the result from \cite{li2023on} and combining it with the result from \cite{barzilai2023generalization}. (See the upper right corner in Table \ref{tab:over_parameterized} or \ref{tab:over_parameterized:2} and Figure \ref{fig:phase_diagram} for visualization.)
For a detailed explanation of our improvements, refer to our novel Proposition \ref{proposition:bias:ub:asymptotic:ridgeless} and the known Proposition \ref{proposition:bias:ub:asymptotic:ridgeless:0} from \cite{barzilai2023generalization} in Section \ref{section:proof}. 




\subsection{Under-parameterization} \label{subsection:under_param}
As illustrated in the flowchart in Figure \ref{fig:flowchart}, the Master inequalities can also provide upper bounds in the under-parameterized setting, which may not be tight. However, obtaining tight bounds in this scenario has a relatively straightforward alternative: when the sample size $n$ tends to infinity with $p<p(n)$, the empirical covariance matrix $\hat{\Si}$  
\begin{equation} \label{line:covariance:convergence}
    \hat{\Si}\to\Si\in\R^{p\times p}
\end{equation}
converges to the population covariance matrix $\Si$ in the operator norm. This convergence allows for the direct application of tight bound techniques, as demonstrated in \cite{cheng2023theoretical}, across all under-parameterized settings. 

In contrast, in the over-parameterized regime, the convergence indicated in line (\ref{line:covariance:convergence}) is only point-wise. This limitation arises because it's impossible to adequately control $p$ independent features with only $n<p$ random samples. Consequently, additional techniques, such as the Master inequalities, are necessary for test error analysis in the over-parameterized regime.

\subsection{Lower bound of test error} \label{subsection:lb}

It is of theoretical interest to provide lower bounds as well. For independent features, we are able to prove that the upper bound is tight using the result from \cite{tsigler2023benign}, generalizing the result from \cite{cui2021generalization}. However, for generic features, we can only provide lower bounds in some but all settings, using the result from \cite{li2023on}. We note that there is some KRR literature, like \cite{li2023on, misiakiewicz2024nonasymptotic, gavrilopoulos2024geometrical}, about matching upper and lower bounds of test error under more assumptions, which is beyond the scope of this paper. For a comparison of assumptions in different papers, see Section \ref{section:assumptions}.




